Modeling Network-level Traffic Flow Transitions on Sparse Data

Modeling how network-level traffic flow changes in the urban environment is useful for decision-making in transportation, public safety and urban planning. The traffic flow system can be viewed as a dynamic process that transits between states (e.g., traffic volumes on each road segment) over time. In the real-world traffic system with traffic operation actions like traffic signal control or reversible lane changing, the system's state is influenced by both the historical states and the actions of traffic operations. In this paper, we consider the problem of modeling network-level traffic flow under a real-world setting, where the available data is sparse (i.e., only part of the traffic system is observed). We present DTIGNN, an approach that can predict network-level traffic flows from sparse data. DTIGNN models the traffic system as a dynamic graph influenced by traffic signals, learns the transition models grounded by fundamental transition equations from transportation, and predicts future traffic states with imputation in the process. Through comprehensive experiments, we demonstrate that our method outperforms state-of-the-art methods and can better support decision-making in transportation.

==> acknowledgments.tex <==
\section{ACKNOWLEDGMENTS}

The work was supported in part by NSF award \#2153311. The views and conclusions contained in this paper are those of the authors and should not be interpreted as representing any funding agencies. 
This research was partially supported by the MOE Innovation Research Team No. IRT\_17R86.

==> redefine.tex <==

\newcommand{\nop}[1]{}
\newcommand{\Todo}{{\textbf{\color{red}{todo-}}}}

\newcommand{\methodFont}{\textsl}
\newcommand{\ours}{\methodFont{the proposed method}\xspace}

%% NOTE that a single column version may be required for 
%% submission and peer review. This can be done by changing
%% the \doucmentclass[...]{acmart} in this template to 
%% \documentclass[manuscript,screen]{acmart}
%% 
%% To ensure 100% compatibility, please check the white list of
%% approved LaTeX packages to be used with the Master Article Template at
%% https://www.acm.org/publications/taps/whitelist-of-latex-packages 
%% before creating your document. The white list page provides 
%% information on how to submit additional LaTeX packages for 
%% review and adoption.
%% Fonts used in the template cannot be substituted; margin 
%% adjustments are not allowed.
